Learning High-Frequency Functions Made Easy with Sinusoidal Positional Encoding

Fourier features based positional encoding (PE) is commonly used in machine learning tasks that involve learning high-frequency features from low-dimensional inputs, such as 3D view synthesis and time series regression with neural tangent kernels. Despite their effectiveness, existing PEs require manual, empirical adjustment of crucial hyperparameters, specifically the Fourier features, tailored to each unique task. Further, PEs face challenges in efficiently learning high-frequency functions, particularly in tasks with limited data. In this paper, we introduce sinusoidal PE (SPE), designed to efficiently learn adaptive frequency features closely aligned with the true underlying function. Our experiments demonstrate that SPE, without hyperparameter tuning, consistently achieves enhanced fidelity and faster training across various tasks, including 3D view synthesis, Text-to-Speech generation, and 1D regression. SPE is implemented as a direct replacement for existing PEs. Its plug-and-play nature lets numerous tasks easily adopt and benefit from SPE.

==> encoding.tex <==
\section{Adaptive Frequency Positional Encoding}\label{encoding}

\begin{figure}[t]
% \centering
\centering
\includegraphics[width=0.45\textwidth]{img/FineNeRF_Encoding.pdf} 
\vspace{-1em}
\caption{Using periodic activation function for Frequency Encoded series.}
\label{fig:encoding}
\end{figure}

Perceptron is the fundamental building block general neural network such as NeRF~\citep{mildenhall2021nerf}, and it is defined as 
\begin{equation}\label{eq:fully-connected}
    \mathbf{y}(\mathbf{x},\mathbf{W}',\mathbf{b}) = g(\mathbf{W}'\cdot\mathbf{x}+\mathbf{b})
\end{equation}

Here $\mathbf{y}\in \mathbb{R}^{d_{out}}$ is the perceptron's output, $g(\cdot)$ is the activation function (usually non-linear), $\mathbf{x}\in\mathbb{R}^{d_{in}}$ is the input, $\mathbf{W}'\in\mathbb{R}^{d_{in}\times d_{out}}$ is the weight matrix, and $\mathbf{b}\in\mathbb{R}^{d_{out}}$ is the bias vector. When $g(\cdot)$ is the identity function and apply a Fourier mapping to the input we get 

\begin{equation}\label{eq2}
    \mathbf{y}(\mathbf{x},\mathbf{W}) = \mathbf{W}\cdot\gamma(\mathbf{x}+\mathbf{b})
\end{equation}

where $\gamma(\cdot)$ is the Fourier mapping defined as 
\begin{equation}\label{eq3}
    \gamma(\mathbf{x}) = [\cos(2\pi\mathbf{B}\cdot\mathbf{x}),\sin(2\pi\mathbf{B}\cdot\mathbf{x})]
\end{equation}

$\mathbf{W}\in\mathbb{R}^{d_{out}\times2m}$, $\mathbf{B}\in\mathbb{R}^{m\times d_{in}}$ is the Fourier mapping matrix, and $m$ is the number of frequencies. Equation~\ref{eq2} is the general equation of a Fourier mapped perceptron. 

The encoding method as stated in Equation~\ref{eq2} is the default positional encoding method in NeRF, where the neural network of NeRF can be simplified by

\begin{equation}\label{eq:nerf-pe}
    \text{NeRF}(\mathbf{x}) = \mathbf{W}
    \begin{bmatrix}
    \sin(\pi\mathbf{x})\\
    \cos(\pi\mathbf{x})\\
    \vdots\\
    \sin(2^{L-1}\pi\mathbf{x})\\
    \cos(2^{L-1}\pi\mathbf{x})\\
    \end{bmatrix}
    + \mathbf{b}
\end{equation}

As Equation~\ref{eq4} indicates, in typical NeRF, the function $\gamma(\cdot)$ would be sequence of mapping
\begin{equation}\label{eq5}
    \gamma({\mathbf{x}}) = [\gamma_0{\mathbf{x}}, \gamma_1{\mathbf{x}}, \cdots, \gamma_{L-1}{\mathbf{x}}]^\mathsf{T}
\end{equation}
The matrix $\mathbf{B}$ need to be properly configured with $2L$ components, representing frequencies to fit the scene representations. Fine tuning $L$ becomes a issue when using NeRF because this is a empirical value varies between scenes.

For frequency domain representation, another alternative is SIREN~\citep{sitzmann2020implicit}. As the previous work~\citep{benbarka2022seeing} indicates that SIREN introduces structurally similar effect as in Equation~\ref{eq3} and \ref{eq4} with trainable parameters, we have

\begin{equation}\label{eq6}
    \mathbf{y}(\mathbf{x},\mathbf{W}) = \mathbf{W}\cdot \sin(2\pi\mathbf{C}\cdot\mathbf{x}+\phi)+\mathbf{b}
\end{equation}
where $\phi := (\pi/2, \dotsc,\pi/2,0, \dotsc,0)^\mathsf{T}\in \mathbb{R}^{2m}$ and $\mathbf{C} := (\mathbf{B},\mathbf{B})^\mathsf{T}$. Here $\mathbf{C}$ acts as the weight matrix applied to the input, $\phi$ as the first bias vector, and $\sin(\cdot)$ is the activation function. The difference is that in SIREN both $\mathbf{C}$ and $\phi$ are trainable. Although Equation~\ref{eq6} shows SIREN has basic adaptive capability on matrix $\mathbf{B}$, it does not resolve the configuration of $L$. By default, SIREN does not give multiple frequency components, \emph{i.e.}, by SIREN itself it cannot carry out a multiple-frequency decomposition as PE.

To effectively merge the advantages of Positional Encoding (PE) and SInusoidal REpresentation Networks (SIREN) in frequency representation, we introduce a novel and efficient method named \textbf{S}inusoid \textbf{P}ositional \textbf{E}ncoding (\textbf{SPE}). The architecture of SPE is depicted in Figure~\ref{encoding}. Our approach involves a simple yet impactful modification: replacing the initial ReLU activation with a SIREN immediately following the PE. Building upon Equations \ref{eq:fully-connected} and \ref{eq:nerf-pe}, SPE can be expressed as follows:
\begin{align}\label{eq:SPE}
\mathbf{y}(\mathbf{x},\mathbf{W}) &= \sin(\mathbf{W} [\sin(\pi x), ..., \cos(2^{L-1}\pi x)] + \bm{\phi}) + \mathbf{b}
\end{align}
In this formulation, $[\sin(\pi x), ..., \cos(2^{L-1}\pi x)]$ represents the positionally encoded input vector comprising $L$ terms. Here, $\mathbf{W}$ and $\bm{\phi}$ denote the learnable weights vector and bias vector of the fully connected layer, respectively. The outer function $\sin(\cdot)$ is applied to each of the element from the output of this layer, and $\mathbf{b}$ signifies an additional bias vector.

Following Equation \ref{eq:SPE}, we have three key observations. First, unlike traditional positional encoding as described in Equation \ref{eq:nerf-pe}, where the number of terms $L$ is a pre-determined hyperparameter, our fully connected layer weights $\mathbf{W}$ inherently attenuate the amplitudes of less significant frequency bands. This unique feature allows our model to naturally circumvent overfitting to unnecessary frequency bands, which is a common issue when $L$ is not optimally set. Second, the inner learnable bias term $\phi$ functions as a phase shift mechanism, dynamically adapting to varying requirements for phase shifting along the x-axis. This adaptability enhances the model's responsiveness to different data characteristics. Third, the integration of an additional SINE layer following the fully connected layer enables SPE to revert to the original PE, as outlined in Equation \ref{eq:nerf-pe}. This design, illustrated in Figure \ref{fig:encoding}, ensures a lower-bounded performance. In essence, it guarantees that SPE's effectiveness will be at least equivalent to, if not better than, that of the traditional PE. This flexibility ensures that the neural network can optimize its performance based on the specific demands of the task at hand.

Next, we will demonstrate two key aspects: Firstly, we will illustrate how SPE can be reduced to PE, thereby ensuring a lower-bound performance that is at least on par with the PE utilized in NeRF, as detailed in Equation \ref{eq:nerf-pe}. Secondly, we will explore how SPE facilitates dynamic frequency feature adaptation, highlighting its capability to adjust to varying data characteristics.

\subsection{Reducing SPE to PE for Guaranteed Lower-Bound Performance}
One of the pivotal features of SPE is its ability to revert to traditional Positional Encoding (PE), which in our architecture depicted in Fig. \ref{fig:encoding}, SPE can be reduced to PE followed by two fully connected layers and ReLU. Without loss of generality, we can focus on one of the terms from positional encoding from Equation \ref{eq:SPE},
\begin{equation}\label{eq:SPE-simplified-1}
    \sin(w (\sin(\alpha x) + \phi) + b
\end{equation}
where $w$ is the learned weight for the current term of $sin(\alpha x)$, $\alpha$ is an element from $\{\pi, ..., 2^{L-1}\pi\}$. Specifically, it can be proved that when $w$ is 1 and we ignore bias term $\phi$ and $b$ (assuming they learned to be 0), Equation \ref{eq:SPE-simplified-1} is structural similar to,
\begin{equation}\label{eq:SPE-simplified-2}
    \sin(1) \sin(\alpha x)
\end{equation}
To prove the marginal difference between Equations \ref{eq:SPE-simplified-2} and \ref{eq:SPE-simplified-1} in special case, we use the Taylor series expansion of the sine function. We apply Taylor expansion to Equation \ref{eq:SPE-simplified-2}, we get,
\begin{align} \label{eq:SPE-taylor}
    \sin(\alpha x) - \frac{\sin(\alpha x)^3}{3!} + \frac{\sin(\alpha x)^5}{5!} + ... \nonumber \\
    &=
    \sin(\alpha x) - \frac{\sin(\alpha x)^3}{3!}
\end{align}
For Equation \ref{eq:SPE-simplified-1} special case, we have
\begin{equation} \label{eq:PE-taylor}
    \sin(1) \left( x - \frac{x^3}{3!} + O(x^5) \right).
\end{equation}
Comparing Equations \ref{eq:SPE-taylor} and \ref{eq:PE-taylor}, we observe that the leading terms differ only by constant coefficients. Therefore, the difference between SPE and PE is marginal for small values of \(x\).

as employed in Neural Radiance Fields (NeRF) \citep{mildenhall2021nerf}. This capability is crucial in ensuring that SPE does not underperform compared to the established PE benchmark. To elucidate this, we refer to the formulation of SPE presented in Equation \ref{eq:SPE}. The architecture of SPE, depicted in Figure \ref{encoding}, involves replacing the initial ReLU activation with a SINE following the PE. This modification, while simple, allows SPE to adapt its functionality.

In scenarios where the complexity introduced by SPE is unnecessary, the network can reduce the SPE to a basic form of PE. This reduction is facilitated by the adjustable weights $\mathbf{W}$ bias $phi$ in the fully connected layer of SPE. When these parameters align to mimic the traditional PE (as outlined in Equation \ref{eq:nerf-pe}), SPE's performance becomes equivalent to that of PE. This ensures a lower-bound performance level where SPE can match, if not exceed, the effectiveness of traditional PE used in NeRF models.

\subsection{Dynamic Frequency Feature Adaptation in SPE}

The second significant aspect of SPE is its ability to enable dynamic frequency feature adaptation. This quality stems from the inherent properties of the SIREN layer integrated into SPE. The sinusoidal activation functions within this layer allow SPE to adapt its response to various frequency components present in the input data.

The key to this adaptability lies in the network's capability to learn and adjust the amplitudes of different frequency bands via its weights $\mathbf{W}$ This is a departure from traditional PE, where the number of terms $L$ is fixed and does not allow for such dynamic adaptation. The learnable bias term $phi$ further contributes to this flexibility, acting as a phase shift mechanism that can dynamically adjust to the requirements of the input data.

This dynamic frequency feature adaptation is particularly beneficial in complex data environments where the input data's frequency characteristics are diverse and non-uniform. By allowing the network to focus on the most relevant frequency components and phase shifts, SPE enhances the overall model's efficiency and accuracy in representing and processing the input data.

% We can observe few features of Equation~\ref{eq7}. Suppose the following layers work with ReLU as activation

% \begin{equation}\label{eq8}
% \mathbf{y}(\mathbf{x},\mathbf{W}) = \begin{cases}
%  \mathbf{W}\cdot \sin(\mathbf{C}\cdot\mathbf{B}\cdot\mathbf{x}+\phi)+\mathbf{b}&\text{$|\mathbf{C}|\geq 1$}\\
%  \mathbf{W}\cdot \mathbf{c} \cdot \sin(\mathbf{B}\cdot\mathbf{x}+\phi)+\mathbf{b}&\text{$|\mathbf{C}| < 1$}
% \end{cases}
% \end{equation}

% where $\mathbf{c}$ is 

* Prove $\mathbf{C}$ can converge through training.

* Prove why 

* Why we still use PE? Because then it is a 2D to 2D task, modifying the frequency is easier than generating from no where

* We should discuss whether the SIREN is only option, or we can use other periodic functions as well. Such as Se ReLU.

* SIREN tends to mimic the input distributions of pixels, empirically SIREN networks is hard to achieve good generalization for new view. We might add more insights here.

\begin{figure}[t]
% \centering
\centering
\includegraphics[width=0.45\textwidth]{img/sin_sin.pdf} 
\vspace{-1em}
\caption{Activation function for Frequency Encoded series.}
\label{fig:sin_sin}
\end{figure}

\begin{figure}[t]
% \centering
\centering
\includegraphics[width=0.45\textwidth]{img/sin_high.pdf} 
\vspace{-1em}
\caption{Activation function for Frequency Encoded series.}
\label{fig:sin_high}
\end{figure}

\begin{figure}[t]
% \centering
\centering
\includegraphics[width=0.45\textwidth]{img/sin_cos.pdf} 
\vspace{-1em}
\caption{Activation function for Frequency Encoded series.}
\label{fig:sin_cos}
\end{figure}









==> evaluation.tex <==
\section{Evaluation}\label{eval}
\begin{table}
\centering
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{l|ccc}
\toprule
Method & PSNR & SSIM  & LPIPS \\
\midrule
 &  &  & \\
\midrule
 &  &  & \\
\midrule
 & & &   \\
\midrule
 &  & & \\
\bottomrule
\end{tabular}%
}
\caption{Evaluation of Different Method.}
\label{table:compare}
\end{table}

\begin{figure}[t]
% \centering
\centering
\includegraphics[width=0.45\textwidth]{img/relative_wasserstein_distance_error.pdf} 
\vspace{-1em}
\caption{Relative Wasserstein Distance Error}
\label{fig:RWDE}
\end{figure}


\begin{figure}[t]
% \centering
\centering
\includegraphics[width=0.45\textwidth]{img/MicrosoftTeams-image (8).png} 
\vspace{-1em}
\caption{GroundTruth}
\label{fig:gtspeech}
\end{figure}

\begin{figure}[t]
% \centering
\centering
\includegraphics[width=0.45\textwidth]{img/MicrosoftTeams-image (9).png} 
\vspace{-1em}
\caption{FastSpeech}
\label{fig:fastspeech}
\end{figure}

\begin{figure}[t]
% \centering
\centering
\includegraphics[width=0.45\textwidth]{img/MicrosoftTeams-image (7).png} 
\vspace{-1em}
\caption{Ours}
\label{fig:ourspeech}
\end{figure}

\begin{figure}[t]
% \centering
\centering
\includegraphics[width=0.42\textwidth]{img/details1.pdf} 
\vspace{-1em}
\caption{Details of Speech Spectrum: High Frequency Details.}
\label{fig:details1}
\end{figure}

\begin{figure}[t]
% \centering
\centering
\includegraphics[width=0.42\textwidth]{img/details2.pdf} 
\vspace{-1em}
\caption{Details of Speech Spectrum: Low Frequency Details.}
\label{fig:details2}
\end{figure}

\begin{figure}[t]
% \centering
\centering
\includegraphics[width=0.49\textwidth]{img/chair.pdf} 
\vspace{-1em}
\caption{Blender Chair $\rightarrow$ wavelet}
\label{fig:chairoverview}
\end{figure}

\begin{figure}[t]
% \centering
\centering
\includegraphics[width=0.49\textwidth]{img/spewavenerf.png} 
\vspace{-1em}
\caption{SPE wavelet}
\label{fig:chairwaveletspe}
\end{figure}

\begin{figure}[t]
% \centering
\centering
\includegraphics[width=0.49\textwidth]{img/freenerfwavelet.png} 
\vspace{-1em}
\caption{FreeNeRF wavelet}
\label{fig:chairwaveletfree}
\end{figure}


==> infoloss.tex <==
\section{High Frequency Information Loss}\label{loss}
On the analysis on the actual frequency and temporal domain gain during learning. Also mention our naive solution here. Add audio as a side example.

\subsection{Level-$\lambda$ Frequency Power}
We conduct wavelet decomposition with $\lambda$ levels on image to separate the high frequency details. Level-$\lambda$ Frequency Power is defined as the power at signal at the $\lambda th$ level decomposition.

\subsection{Naive NeRF baseline with Formal Method}


\subsection{Gain of New View Generation}

==> metrics.tex <==
\section{Metrics}
\subsection{High Frequency Information Loss}\label{loss}
On the analysis on the actual frequency and temporal domain gain during learning. Also mention our naive solution here. Add audio as a side example.

\subsubsection{Level-$\lambda$ Frequency Power}
We conduct wavelet decomposition with $\lambda$ levels on image to separate the high frequency details. Level-$\lambda$ Frequency Power is defined as the power at signal at the $\lambda th$ level decomposition.

\subsubsection{Gain of New View Generation on High Frequency Details}

\subsection{Relative Wasserstein Distance Error}

\subsection{Commonly Used Metrics in Different Tasks}


==> practice.tex <==
\section{Sinusoidal Positional Encoding in Practice}\label{sec:implementation}
% \subsection{Implementation of SPE}\label{sec:implementation}
\begin{figure}[t]
% \centering
\centering
\includegraphics[width=0.45\textwidth]{img/FineNeRF_Encoding.pdf} 
\vspace{-1em}
\caption{Using periodic activation function for Frequency Encoded series.}
\label{fig:encoding}
\end{figure}

In this section, we discuss different concerns we addressed while implementing SPE. For a given network, we replace the first activation function after PE with a sinusoidal activation. We illustrate this using an SPE-enabled NeRF in Figure~\ref{fig:encoding}. The addition of SPE does not change the training process, making SPE easy to adopt in existing neural networks. 

\textbf{Theorem 3.} $L$ determines the approximation accuracy of SPE to a trainable PE (proof in \S\ref{spelearn}).
\begin{equation}
\sin(\omega\text{PE}(\mathbf{x})) = \text{PE}(\omega(\mathbf{x}+\frac{1}{2^L}))
\end{equation}

The only hyper-parameter of SPE is the $L$. 
Since Fourier feature $\omega$ is trainable, the value $L$ in PE is the larger the better and should match the network size, $L \propto N_{\text{para}}$ where $N_{\text{para}}$ is the number of parameters in the network. Using larger $L$ should not cause unexpected artefacts because the features in the PE part will be tuned by $\omega$. In our experiments, we can optimize $L$ by increasing the number until the result does not improve.

\subsection{Choice of learning methods}\label{sec:altlearn}

We first discuss the choice of learning methods together with SPE.
One option is to learn $\sin(\omega\mathbf{x})$ directly as in Equation~\ref{eq:ape}. Compared with learning in a form $\sin(\omega\mathbf{x})$, Incorporating PE with SPE simplifies training by limiting the search to a bounded space, unlike other methods that operate in a larger, unbounded space. This constraint leads to more stable training and faster convergence.

Suppose we have $L$ components in SPE, then the hardcoded features is $\mathbf{f}_{h} =[\pi, 2\pi, \dots, 2^{L-1}\pi]$, and the learned features (suppose the actual features is distinct to the hardcoded features) $\mathbf{f}_{l} =[\omega_0\cdot\pi, \omega_1\cdot2\pi, \dots, \omega_L\cdot2^{L-1}\pi]$. Assume that the actual feature is $\omega_a$, the difference between the nearest hardcoded feature and actual feature $\Delta_{\text{PE}}$ would be
\begin{align}\label{pebound}
    \begin{cases}
\Delta_{\text{PE}} = \min(2^{\beta_0}\pi - \omega_a,\omega_a - 2^{\beta_1}\pi) & \omega_a < 2^{L-1}\pi\\
\Delta_{\text{PE}} = \omega_a - 2^{L-1}\pi & \omega_a \geq 2^{L-1}\pi
\end{cases}
\end{align}

Where $\beta_0 = \lceil\log_2\frac{\omega_a}{\pi}\rceil$ and $\beta_1 = \lfloor\log_2\frac{\omega_a}{\pi}\rfloor$. Therefore if we have PE, then tuning the frequency always can be converted to a bounded range that is significantly smaller than $\omega_a$ when $L$ is large enough. Without embedding PE in SPE, the searching space to train $\omega$ is not bounded and will be sensitive to initialization, which is hard to carry out when the actual feature is unknown.  

\subsection{Choice of periodic activation functions}

We next discuss which periodic activation functions shall be used in SPE. Accordinbg to the Fourier theorem, any continuous series can be expanded as a combination of sinusoidal waves, therefore representing sinusoidal waves is critical to guarantee that all target output can be correctly presented. Basically, to make sure the network can represent the sinusoidal wave, condition \ref{approxtarget0} must be met, otherwise the rest of the network after SPE has to learn a weight that is conditional on the Fourier features, which makes the learning more difficult. For instance, if there is significant linear mapping in the activation, then $\mathbf{I}(\cdot)$ or $\mathbf{S}(\cdot)$ will have a form (proof in \S\ref{otheract}), where each feature has to be learned in coupling with specific input $\mathbf{x}$.
\begin{equation}\label{eqst_0}
    \mathbf{S}(t) = \frac{\sin(\mathbf{W}_{\text{SPE}}\cdot t)}{\sqrt{\mathbf{W}_{\text{SPE}}^2-(2n\pi)^2} \bmod 2\pi}
\end{equation}
Where $\mathbf{W}_{\text{SPE}} = [\omega_0, \dots, \omega_L]$. The function in Equation~\ref{eqst_0} is much harder to learn than Equation~\ref{IS_0} and \ref{IS_1}, potentially representing wrong frequency features for $\mathbf{x}$ that is not in the training set. Therefore we propose using sinusoidal activation.

\subsection{Choice of encoding methods}\label{hashreasoning}

We finally compare different encoding methods: One Blob Encoding and Hash Encoding~\citep{muller2022instant}. While claiming faster training, we find that the One Blob Encoding based method shows much worse performance than the PE or SPE-based method in few-view NeRF.

Instead of using sinusoidal functions, in Hash encoding the input $\mathbf{x}$ is encoded by hashing~\citep{muller2022instant}
\begin{equation} \label{eq:hash-encoding}
   h(\mathbf{x}) =  (\bigoplus^d_{i=1}x_i\pi_i) \mod T
\end{equation}
where $\oplus$ denotes the bit-wise XOR operation and $\pi_i$ are unique,
large prime numbers. If look from PE point of view, Hash encoding using a pseudo random function~\citep{muller2019neural} to replace the sinusoidal function, \emph{i.e.}, Fourier features of PE. Essentially, since there are multiple Hash tables, Hash encoding essentially performs a Monte-Carlo search for proper encoding. Then the model needs to learn from the encoding to match actual features. 

When using Hash encoding, there will be a Hash collision, where different $x_i$ might be mapped into the same value in a pseudo-random manner. In the implementation with MLP, such as InstantNeRF~\citep{muller2022instant} and NeRFfacto~\citep{tancik2023nerfstudio}, they do not explicitly handle collisions of the hash functions by typical means like probing, bucketing, or chaining. Instead, we rely on the neural network to
learn to disambiguate hash collisions themselves, avoiding control flow divergence, reducing implementation complexity and improving performance. 

Through an experiment in \S\ref{subsec:nerf}, we find that NeRF with Hash encoding on a small number of training views performs much worse than SPE in terms of fidelity. Both searching for appropriate encoding and learning to fix Hash collision requires lots of effective inputs (\emph{i.e.}, distinct views in NeRF), and hence it is hard to train NeRF with Hash encoding on limited views. 

In summary, although Hash encoding has a significant advantage in terms of computation (training time), the learning efficiency, \emph{i.e.}, and the ability to extract appropriate features, are much worse than SPE.

==> wd.tex <==
\section{Training Method}\label{training}
\subsection{Training of SPE}\label{trainspe}
To train the SPE layer, we follow the same initialization as \cite{sitzmann2020implicit}. We differ our task from the SIREN networks in \cite{sitzmann2020implicit}, where the task is to learn the information hidden in $n$-th order difference of the original data. We only use one layer of SIREN to learn a proper frequency representation, hence there is no specific limitation on the following layers, such as the implmentation for NeRF in Figure~\ref{encoding}.

\subsection{Minimizing Wasserstein Distance Error in NeRF}\label{wd}
We use a training trick during training NeRF with SPE. As earlier work shows[], in general GANs help learning high frequency details, which helps the training of the high frequency decomposition as well.

We find in NeRF, the earth moving distance actually matches the process of the moving of pixels. Although with distortion, the distribution shift of the pixels is actually condition on the viewpoint. We demonstrate this by an example in Figure. Therefore for the training of NeRF, we follow the procedure in \cite{arjovsky2017wasserstein}. For more reasoning see Appendix~\ref{appendix:EMD}.
% \subsection{Second Chance: Synthetic View Selection}
% We propose a method to select best fidelity output from multiple versions. 

% Hints - 

% (1) See image as a distribution of pixel, near view should have very close EMD, even after rotation. 

% (2) Some local feature should be clear and easy to identify. But it might be challenging to find the latent feature.

% (3) Blurring, Contrast, and model uncertainty.

% \subsection{Optional: Nearest Scene and Interpolation}
% We formulate a naive NeRF method without learning process to perform as a baseline.

% Instead of doing NeRF, we model new view generation task as a frame interpolation process.

% We get the new view by interpolating based on nearest $n$ views. 

% Essentially, we formulate the new view generation as an optimization problem. 
